Probing Reionization with Quasar Spectra: the Impact of the Intrinsic Lyman-alpha Emission Line Shape Uncertainty

Arguably the best hope of understanding the tail end of the reionization of the intergalactic medium (IGM) at redshift z > 6 is through the detection and characterization of the Gunn-Peterson (GP) damping wing absorption of the IGM in bright quasar spectra. However, the use of quasar spectra to measure the IGM damping wing requires a model of the quasar's intrinsic Lyman-alpha emission line. Here we quantify the uncertainties in the intrinsic line shapes, and how those uncertainties affect the determination of the IGM neutral fraction. We have assembled a catalog of high-resolution HST spectra of the emission lines of unobscured low-redshift quasars, and have characterized the variance in the shapes of their lines. We then add simulated absorption from the high-redshift IGM to these quasar spectra in order to determine the corresponding uncertainties in reionization constraints using current and future samples of z > 6 quasar spectra. We find that, if the redshift of the Lyman-alpha emission line is presumed to coincide with the systemic redshift determined from metal lines, the inferred IGM neutral fraction is systematically biased to low values due to a systematic blueshift of the Lyman-alpha line relative to the metal lines. If a similar blueshift persists in quasars at z > 6, this bias strengthens previous claims of a significant neutral hydrogen fraction at z ~ 6. This technique is capable of making a robust distinction between a highly ionized (x_IGM ~ 10^-3) and a neutral (x_IGM = 1) IGM with even a few bright quasars.

==> table1.tex <==
MRK 0335&0.026&FOS&B-3&H13&  16.2&Fit with free line centers flags a large number of pixels as
"emission" features.\\
FAIRALL 0009&0.047&FOS&B-3&H13&  10.8&                            Excluded due to non-convergence of feature detection.\\
UGC 00545&0.061&FOS&B-3&H13&  25.6&                            Excluded due to non-convergence of feature detection.\\
UGC 11763&0.063&HRS&LSA&G140L&  20.5&                            Excluded due to non-convergence of feature detection.\\
MR 2251-178&0.064&FOS&B-3&H13&  14.3&                            Excluded due to non-convergence of feature detection.\\
TON 1187&0.079&FOS&B-3&H13&  11.0&             Feature detection did not converge for red-side fit with zero shift.\\
MRK 0478&0.079&FOS&B-3&H13&  11.6&                    Excluded due non-convergence of feature detection (all fits).\\
PG 1211+143&0.081&FOS&B-3&H13&  11.2&                            Excluded due to non-convergence of feature detection.\\
PG 1211+143&0.081&HRS&LSA&G140L&  26.7&                            Excluded due to non-convergence of feature detection.\\
SDSS J12305003+0115226&0.117&HRS&LSA&G140L&  25.0&Excluded due to feature detection non-convergence (and many absorption
features).\\
SBS 1626+554&0.133&FOS&B-3&H13&  10.5&                                        Strong absorption feature at line center.\\
PG 0026+129&0.142&FOS&B-3&H13&  15.0&Full fit spuriously excludes a large region on red side as absorption,
but fits well on the blue side of the line.\\
PG 1114+445&0.144&FOS&B-3&H13&  12.7&                            Excluded due to non-convergence of feature detection.\\
  3C 273&0.158&FOS&C-2&H13&  20.9&                                                                                 \\
  3C 273&0.158&FOS&B-2&H13&  19.9&                                                                                 \\
  3C 273&0.158&FOS&B-3&H13&  17.6&                                                                                 \\
  3C 273&0.158&FOS&A-1&H13&  17.0&                                                                                 \\
  3C 273&0.158&FOS&B-1&H13&  18.1&                                                                                 \\
PG 1322+659&0.168&FOS&B-3&H13&  18.0&      Full fit excludes a large section of blue side contaminated with ISM lines.\\
PG 1116+215&0.176&FOS&C-2&H13&  15.9&                                                                                 \\

[HB89] 1427+480&0.221&FOS&B-3&H13&  12.8&               Absorption feature in blue wing of the line (flagged in full fit).\\
PG 0953+414&0.234&FOS&C-2&H13&  11.1&                                               Absorption feature at line center.\\

[HB89] 1156+213&0.349&FOS&B-3&H19&  10.7&                                                                                 \\
PG 1049-005&0.360&FOS&C-2&H19&  13.6&                                       Excluded due to bad blue edge of spectrum.\\

[HB89] 1425+267&0.366&FOS&B-3&H19&  12.5&                             Strong absorption line just blueward of line center.\\
HS 0624+6907&0.370&FOS&B-2&H19&  17.2&                                                                                 \\
SBS 1704+608&0.372&FOS&C-2&H19&  13.9&                                       Excluded due to bad blue edge of spectrum.\\

[HB89] 1543+489&0.400&FOS&B-3&H19&  27.4&   Highly asymmetric profile. Red-side fit with median shifts failed to
converge.\\
  3C 215&0.412&FOS&A-1&H19&  11.7&                                                                                 \\
LBQS 1230+0947&0.414&FOS&A-1&H19&  10.3&                                                                                 \\

[HB89] 1049+616&0.421&FOS&C-1&L15&  13.4&                                                                                 \\

[HB89] 2308+098&0.433&FOS&B-3&H19&  17.4&                                                                                 \\
PG 0003+158&0.451&FOS&C-2&H19&  19.9&                                                                                 \\
FBQS J0745416+314256&0.461&FOS&C-2&H19&  13.3&                                                                                 \\

[HB89] 2112+059 NED01&0.466&FOS&C-2&H19&  13.0&                                                                                 \\
SBS 1259+593&0.478&FOS&C-2&H19&  16.1&                   Poorly constrained very narrow component in all red-side fits.\\

[HB89] 2128-123&0.501&FOS&C-2&H19&  19.9&                       Full profile fit flags red side of the Ly-alpha line core.\\

[HB89] 1130+111&0.510&FOS&C-2&H19&  10.6&                                                   Excluded due to bad blue edge.\\

[HB89] 0850+440&0.514&FOS&C-2&H19&  10.8&                                                                                 \\
FBQS J0958209+322402&0.530&FOS&C-2&H19&  10.9&               Missing some flux values at line center (flagged during coadding).\\

[HB89] 0454-220&0.533&FOS&B-3&H19&  25.1&                            Excluded due to non-convergence of feature detection.\\
TON 0156&0.549&FOS&B-3&H19&  31.6&                                  Excluded due to problems with coadded spectrum.\\

[HB89] 0015+162&0.553&FOS&B-3&H19&  12.5&                                                                                 \\
PG 1333+176&0.553&FOS&C-2&H19&  12.3&                                       Excluded due to bad blue edge of spectrum.\\
  3C 334&0.555&FOS&C-2&H19&  15.0&                                                                                 \\
NGC 2841 UB3&0.556&FOS&C-2&H19&  14.3&                                                                                 \\

[HB89] 1136-135&0.558&FOS&C-2&H19&  11.5&                        Red-side fit spuriously flagged some of narrow component.\\

[HB89] 0405-123&0.573&FOS&C-2&H19&  18.2&                                                                                 \\

[HB89] 0439-433&0.593&FOS&C-2&H19&  14.0&                      Region of red side flagged as emission in full-profile fit.\\
FBQS J1010275+413238&0.612&FOS&C-2&H19&  19.9&                                                                                 \\
  3C 095&0.616&FOS&C-2&H19&  17.2&                                                                                 \\
PG 0044+030&0.623&FOS&C-2&H19&  10.8&                                                                                 \\

[HB89] 1104+167&0.632&FOS&C-2&H19&  17.9&                                                                                 \\

[HB89] 2243-123&0.632&FOS&C-2&H19&  17.2&                                                                                 \\
  3C 263&0.646&FOS&A-1&H19&  10.2&                                                                                 \\
  3C 263&0.646&FOS&C-2&H19&  14.2&                                                                                 \\
  3C 057&0.669&FOS&B-2&H19&  25.2&                                                                                 \\

[HB89] 2344+092&0.677&FOS&C-2&H19&  12.5&               Full fit flags edges of the narrow component as emission features.\\

[HB89] 0923+392&0.695&FOS&A-1&H19&  21.1&                                                                                 \\

[HB89] 2352-342&0.702&FOS&C-2&H19&  15.8&                        Red edge of narrow component is flagged in red-side fits.\\

[HB89] 1354+195&0.720&FOS&C-2&H19&  11.4&                                                                                 \\
FBQS J1159+2914&0.729&FOS&B-3&H19&  13.5&                       Excluded due to poor signal-to-noise, weak emission lines.\\

[HB89] 1637+574&0.751&FOS&A-1&H19&  10.9&                                                                                 \\

[HB89] 1538+477&0.772&FOS&C-2&H19&  21.7&                                Several absorption features on red and blue side.\\
2MASSi J1003067+681316&0.773&FOS&C-2&H19&  12.3&                            Poorly constrained narrow component in red-side fits.\\
  3C 110&0.775&FOS&B-3&H19&  12.1&                                                                                 \\
FBQS J1253175+310550&0.780&FOS&B-3&H19&  28.9&                                                                                 \\
LBQS 0102-2713&0.780&FOS&B-3&H19&  27.4&                                                                                 \\
  3C 286&0.849&FOS&A-1&L15&  13.2&                                                                                 \\
 3C 4543&0.859&FOS&C-2&H27&  12.0&                        Narrow component poorly constrained in all red-side fits.\\
 3C 4543&0.859&FOS&A-1&H27&  13.4&                                                                                 \\

[HB89] 0107-156&0.861&FOS&B-3&H27&  16.7&                            Narrow component poorly constrained in red-side fits.\\

[HB89] 1252+119&0.873&FOS&C-2&H27&  12.5&                                                                                 \\
LBQS 0253-0138&0.879&FOS&A-1&H27&  10.2&                                                                                 \\

[HB89] 2340-036&0.892&FOS&C-2&H27&  16.0&Lots of bad pixels. Full fit has unconstrained emission component on
red side of line.\\

[HB89] 0954+556&0.896&FOS&A-1&H27&  10.9&                                                                                 \\

[HB89] 2216-038&0.901&FOS&A-1&H27&  14.7&                                                                                 \\
PKS 0823-223&0.910&FOS&B-3&H27&  15.5&                      Excluded due to lack of visible emission lines in spectrum.\\
  3C 336&0.927&FOS&B-3&H27&  13.9&ISM absorption line in center of Ly-alpha line. 
Other prominent absorption features.\\
FBQS J1409239+261821&0.940&FOS&C-2&H27&  15.6&                                             Excluded due to weak emission lines.\\
SBS 1340+606&0.964&FOS&A-1&H27&  12.7&                 Excluded due to strong absorption features (blue- and red-side).\\
  3C 094&0.965&FOS&A-1&H27&  10.9&                     Excluded due to strong absorption lines (red and blue side).\\
TON 0157&0.971&FOS&B-3&H27&  15.6&                                       Negative narrow component in red-side fit.\\
SBS 1148+549&0.975&FOS&A-1&H27&  15.2&                                              Very broad, blended emission lines.\\

[HB89] 2145+067&0.990&FOS&C-2&H27&  10.9&                                                     Highly asymmetrical profile.\\

[HB89] 0355-483&1.016&FOS&A-1&H27&  12.0&                            Narrow component poorly constrained in red-side fits.\\
TON 0153&1.022&FOS&C-2&H27&  16.3&                                                                                 \\
PG 1254+047&1.025&FOS&C-2&H27&  15.6&Narrow component poorly constrained in red-side fit. Red-side fit with
median shifts failed to converge. Very broad blended emission lines.\\
PG 1248+401&1.033&FOS&B-2&H27&  16.1&                                                                                 \\

[HB89] 2230+114&1.037&FOS&A-1&H27&  13.2&                                                                                 \\
LBQS 1229-0207&1.043&FOS&C-1&H27&  17.8&                                                                                 \\

[HB89] 2302+029&1.044&FOS&B-3&H27&  25.0&                              Unusual line shape and lots of absorption features.\\
SBS 1317+520&1.061&FOS&A-1&H27&  12.5&                                                                                 \\

[HB89] 1718+481&1.084&FOS&C-2&H27&  27.5&                                 Several absorption features and many bad pixels.\\

[HB89] 0024+224&1.119&FOS&C-2&H27&  11.9&                                                Narrow absorption in line center.\\
PG 1352+011&1.127&FOS&C-2&H27&  14.0&Several moderate-width absorption features. Poorly constrained very
narrow component in blue-side fits.\\
PG 1206+459&1.163&FOS&C-2&H27&  15.5&                                                 Some narrow absorption features.\\
PG 1338+416&1.214&FOS&C-2&H27&  12.3&                               Excluded due to prominent IGM absorption features.\\
PG 0946+301&1.221&FOS&B-3&H27&  20.7&                               Excluded due to strong, broad absorption features.\\

[HB89] 1038+064&1.270&FOS&B-2&H27&  19.6&                                                 Several narrow absorption lines.\\
PG 1241+176&1.273&FOS&C-2&H27&  20.7&                                       Some narrow blue-side absorption features.\\
PG 1008+133&1.289&FOS&C-2&H27&  17.4&Missing red-side fit with median shifts due to non-convergence of
feature detection.  Many narrow absorption features.\\

[HB89] 1634+706&1.334&FOS&C-2&H27&  45.6&                            Excluded due to non-convergence of feature detection.\\

[HB89] 0454+039&1.345&FOS&C-1&H27&  17.0&                            Excluded due to non-convergence of feature detection.\\

[HB89] 0454+039&1.345&FOS&B-3&H27&  14.3&                                              Lots of narrow absorption features.\\
FBQS J1259487+342322&1.375&FOS&C-2&H27&  12.8&                    Strong narrow absorption feature just redward of line center.\\

[HB89] 0302-223&1.409&FOS&B-1&H27&  23.5&                            Narrow component poorly constrained in red-side fits.\\

[HB89] 0957+561&1.414&FOS&B-1&H27&  44.6&                  Excluded due to strong absorption features (red and blue side).\\
  3C 298&1.437&FOS&B-3&H27&  21.3&              Excluded due to strong, broad absorption lines (red and blue side).\\

[HB89] 0232-042&1.440&FOS&B-2&H27&  24.0&                                                                                 \\
SDSS J12184047+5015434&1.456&FOS&A-1&H27&  24.3&                                             Excluded due to missing flux values.\\
  UM 425&1.462&FOS&B-2&H27&  19.7&            Excluded due to prominent broad absorption lines (red and blue side).\\

[HB89] 1630+377&1.476&FOS&B-1&H27&  28.6&                                                                                 \\
PG 0117+213&1.493&FOS&B-2&H27&  19.6&Many narrow absorption features. Red-side fit has a poorly-behaved
narrow component.\\

[HB89] 0743-673&1.510&FOS&C-2&H27&  22.0&Large section of line spuriously flagged by feature detection in full
fit. Blue side of fit still good.\\
LBQS 1026-0045B&1.531&FOS&B-3&H27&  22.6&                                          Excluded due to misaligned sub-spectra.\\

[HB89] 1115+080&1.735&FOS&B-2&H40&  22.5&                   Excluded due to absorption features (in both Ly-alpha
and NV).\\
CTS 0286&2.545&FOS&B-1&L65&  23.1&                                Excluded due to high redshift and low resolution.\\

[HB89] 1413+117&2.558&FOS&B-1&H40&  20.5&                                       Excluded due to broad absorption features.\\
MAPS-NGP O\_382\_0380226&3.620&FOS&B-2&H57&  24.2&                                   Excluded due to high blue-side IGM absorption.\\


==> table2.tex <==
MRK 0335&FOS H13 B-3&  2.13&  8.48&100&  9.18&  2.80&-258&  4.76&  0.98&24& -1.09&   76.2&  1.24&  0.88&199&177\\
SBS 1626+554&FOS H13 B-3&  4.76&  2.26&-518&  17.1&  1.42&-94&  6.63&  0.49&-156& -1.35&   21.8&  1.27&  1.24&326&217\\
PG 0026+129&FOS H13 B-3&  3.29& 12.22&1824&  14.9&  1.04&694&  5.22&  0.92&1108& -1.06&   19.1&  1.20&  1.26&311&199\\
  3C 273&FOS H13 A-1&  4.48&  1.44&-557&  16.9&  0.68&-169&  6.44&  0.19&283& -1.30&    270&  0.76&  0.79&372&204\\
  3C 273&FOS H13 B-3&  4.25&  1.57&-631&  17.1&  0.68&-135&  7.58&  0.16&102& -1.17&    268&  1.14&  1.08&354&204\\
  3C 273&FOS H13 B-1&  4.18&  1.58&-610&  16.7&  0.67&-491&  7.62&  0.21&39& -1.21&    280&  1.15&  1.04&352&203\\
  3C 273&FOS H13 C-2&  4.14&  1.46&-524&  15.2&  0.71&-523&  7.51&  0.23&66& -1.34&    280&  1.03&  0.88&317&160\\
  3C 273&FOS H13 B-2&   4.1&  1.58&-644&  16.6&  0.70&-250&  7.47&  0.19&245& -1.39&    274&  0.83&  0.82&355&203\\
PG 1322+659&FOS H13 B-3&  3.48&  3.84&-220&  11.5&  2.46&-1007&  5.03&  0.93&-308& -1.25&    9.2&  2.63&  1.51&279&194\\
PG 1116+215&FOS H13 C-2&  4.41&  1.29&-336&  14.2&  1.02&-683&  6.96&  0.48&115& -2.38&   58.7&  0.88&  0.58&362&219\\

[HB89] 1427+480&FOS H13 B-3&  3.54&  3.81&213&  13.5&  1.61&-457&   6.4&  0.56&309& -1.10&    7.8&  1.32&  1.08&350&110\\
PG 0953+414&FOS H13 C-2&  3.76&  3.57&-270&  14.9&  1.85&-112&  5.03&  0.68&225& -0.75&   16.6&  1.35&  0.69&396&110\\

[HB89] 1156+213&FOS H19 B-3&  4.62&  3.03&-510&  17.9&  1.57&-1780&  7.05&  0.56&-470& -1.30&   3.15&  0.87&  0.78&248&156\\

[HB89] 1425+267&FOS H19 B-3&  5.29&  0.91&2228&  14.4&  2.48&-1700&  4.97&  0.61&775& -1.87&   4.01&  1.63&  0.90&271&185\\
HS 0624+6907&FOS H19 B-2&  4.58&  4.13&-786&  13.1&  2.27&-1365&  7.74&  1.42&-823& -1.30&     15&  0.90&  0.76&252&133\\

[HB89] 1543+489&FOS H19 B-3&  2.79&  1.86&-307&  13.7&  2.11&-1578&  7.11&  0.99&-964& -1.23&   5.53&  1.55&  0.99&273&149\\
  3C 215&FOS H19 A-1&  2.98&  2.91&-498&  11.3&  4.07&192&  7.03&  0.76&1019& -3.38&  0.929&  0.65&  0.54&339&197\\
LBQS 1230+0947&FOS H19 A-1&  4.95&  2.88&424&  13.7&  2.40&628&  5.33&  1.44&830& -0.94&   5.86&  1.11&  1.33&337&175\\

[HB89] 1049+616&FOS L15 C-1&  8.51&  0.94&88&  23.2&  0.86&2733&-0.0497&  1.23&967& -2.21&   5.74&  0.98&  0.68&61&39\\

[HB89] 2308+098&FOS H19 B-3&   3.9&  1.27&-130&  11.8&  1.11&-114&  7.68&  0.49&263& -4.20&   7.73&  0.71&  0.57&330&197\\
PG 0003+158&FOS H19 C-2&  2.44&  2.67&-229&  10.4&  2.09&-315&  8.17&  0.45&-380& -2.93&   13.1&  1.28&  0.51&327&202\\
FBQS J0745416+314256&FOS H19 C-2&  2.53&  1.41&-634&  10.8&  1.73&-596&  8.99&  0.50&-951& -4.11&   6.86&  0.84&  0.63&350&214\\

[HB89] 2112+059 NED01&FOS H19 C-2&  3.02&  1.34&-1534&  18.2&  1.20&25&  1.51& -0.06&409& -3.09&   6.97&  0.97&  0.59&351&181\\
SBS 1259+593&FOS H19 C-2&  4.57& -0.20&463&  17.4&  0.83&-879& 0.806& -0.10&-43& -2.69&   12.6&  0.76&  0.85&353&216\\

[HB89] 2128-123&FOS H19 C-2&   5.6&  3.14&-114&  22.8&  1.39&1563& 0.885& -0.16&1696& -1.30&   8.66&  1.76&  1.88&226&178\\

[HB89] 0850+440&FOS H19 C-2&  3.31&  1.10&-26&  8.84&  1.09&-1100&  7.87&  0.44&-717& -4.41&   5.48&  0.43&  0.59&341&191\\
FBQS J0958209+322402&FOS H19 C-2&  4.38&  0.68&-676&  14.7&  0.50&-487&  7.05&  0.24&-124& -3.07&   5.47&  0.32&  0.61&337&224\\

[HB89] 0015+162&FOS H19 B-3&  4.26&  2.28&-720&  22.7&  0.99&117&  3.29&  0.36&-752& -2.22&   0.48&  0.98&  1.09&346&228\\
  3C 334&FOS H19 C-2&  3.27&  0.97&-282&  16.7&  0.95&-478&  8.47&  0.13&663& -3.85&   6.37&  0.89&  1.01&350&227\\
NGC 2841 UB3&FOS H19 C-2&  3.35&  0.71&-841&    13&  1.00&-1645&  7.16&  0.51&-1001& -2.78&   6.73&  1.00&  0.98&352&211\\

[HB89] 1136-135&FOS H19 C-2&  1.98&  3.40&-495&  9.08&  2.13&-209&   6.4&  0.49&-254& -3.69&   5.53&  1.29&  0.92&352&230\\

[HB89] 0405-123&FOS H19 C-2&  2.52&  2.56&-213&  11.2&  1.98&-51&  5.92&  0.65&97& -1.88&   16.6&  1.32&  0.86&336&210\\

[HB89] 0439-433&FOS H19 C-2&   2.6&  3.54&-132&  15.7&  1.00&-471&   6.2&  0.29&493& -3.56&   4.32&  1.39&  0.86&340&224\\
FBQS J1010275+413238&FOS H19 C-2&   3.2&  2.98&-67&  12.9&  2.19&-289&  5.91&  0.86&209& -2.48&   6.97&  2.09&  1.46&338&200\\
  3C 095&FOS H19 C-2&  10.7&  0.71&-40&  26.1&  0.45&3087& 0.277& -0.03&1818& -2.44&   10.1&  0.96&  1.05&355&237\\
PG 0044+030&FOS H19 C-2&  4.11&  1.66&-495&  10.8&  1.38&-2393&  12.5&  1.02&-2019& -3.27&   4.38&  0.69&  0.62&390&238\\

[HB89] 2243-123&FOS H19 C-2&  2.47&  3.02&-1164&  11.9&  1.53&-925&  7.11&  0.36&-528& -3.51&   5.35&  1.69&  0.88&392&239\\

[HB89] 1104+167&FOS H19 C-2&  2.06&  1.80&-571&  9.25&  2.42&-260&  9.77&  0.79&-962& -2.59&   8.39&  1.22&  1.22&365&239\\
  3C 263&FOS H19 A-1&  3.34&  3.48&-120&  13.6&  1.73&250&  4.58&  0.53&328& -1.58&    6.3&  1.22&  1.16&395&242\\
  3C 263&FOS H19 C-2&  2.67&  2.88&-309&  11.5&  1.81&-211&   6.2&  0.49&622& -2.19&   7.62&  1.68&  0.68&374&240\\
  3C 057&FOS H19 B-2&  6.87&  1.46&66&  10.9&  0.50&-4478&  7.53&  0.56&-266& -1.21&   6.85&  2.53&  1.37&376&235\\

[HB89] 2344+092&FOS H19 C-2&  2.52&  5.04&-1037&  15.2&  1.19&-1709&   6.7&  0.48&-983& -3.12&   4.26&  1.42&  1.23&347&237\\

[HB89] 0923+392&FOS H19 A-1&  5.18&  2.23&591&  18.3&  1.34&1163&  5.67&  0.16&779& -0.02&   4.33&  0.97&  1.00&385&189\\

[HB89] 2352-342&FOS H19 C-2&  1.62&  2.91&703&  12.8&  2.27&85&  4.84&  0.49&940& -2.40&   4.89&  1.97&  0.90&339&227\\

[HB89] 1354+195&FOS H19 C-2&  2.04&  4.16&-208&  10.3&  1.90&-175&  5.88&  0.51&-47& -3.58&   4.16&  1.54&  0.89&414&160\\

[HB89] 1637+574&FOS H19 A-1&  3.53&  2.09&-84&    13&  1.10&135&  6.35&  0.48&191& -1.50&   3.04&  1.16&  0.87&422&128\\

[HB89] 1538+477&FOS H19 C-2&  5.92&  1.47&-283&  15.8&  1.96&-148&  6.55&  0.33&917& -1.10&   5.82&  2.42&  1.80&288&112\\
2MASSI J1003067+681316&FOS H19 C-2&  5.19&  0.42&-980&  16.4&  0.59&-2850&  8.19&  0.64&-1616& -3.00&   3.06&  1.11&  1.16&387&111\\
  3C 110&FOS H19 B-3&  2.16&  1.44&-232&  14.4&  1.80&330&   7.4&  0.45&733& -0.53&   4.14&  1.40&  1.19&426&112\\
LBQS 0102-2713&FOS H19 B-3&  3.13&  1.68&-661&  12.2&  2.06&-1699&     8&  0.87&-1268& -2.00&   1.38&  2.24&  2.38&346&75\\
FBQS J1253175+310550&FOS H19 B-3&  7.24&  0.65&-396&  18.2&  1.11&793&  4.84&  0.27&-262& -2.39&   2.87&  3.76&  2.60&335&66\\
  3C 286&FOS L15 A-1&  5.57&  1.08&-1757&  17.9&  0.73&-1000&   3.1&  0.18&-1131& -1.07&   1.77&  1.02&  1.84&75&12\\
 3C 4543&FOS H27 C-2&  2.84&  1.44&-556&  10.5&  0.66&-299&  3.46&  0.28&-255& -1.30&   2.78&  0.62&  0.78&217&146\\
 3C 4543&FOS H27 A-1&  4.22&  2.65&-301&  19.3&  0.56&79&  3.16&  0.32&20& -1.30&   1.59&  1.13&  1.39&212&141\\

[HB89] 0107-156&FOS H27 B-3&  3.53&  2.35&-703&  19.1&  1.56&-604&  3.62&  0.27&-1366& -1.30&   0.73&  1.01&  0.96&191&126\\

[HB89] 1252+119&FOS H27 C-2&  6.34&  1.56&-734&  29.9&  0.42&-1778&  6.39&  0.41&-1002& -1.30&   2.24&  0.90&  0.85&264&155\\
LBQS 0253-0138&FOS H27 A-1&  6.23&  1.07&-399&  9.48&  0.61&-3833&  10.8&  0.72&-1626& -1.30&   2.22&  1.21&  1.34&267&146\\

[HB89] 2340-036&FOS H27 C-2&  4.52&  1.58&205&  16.1&  1.21&440&  9.54&  1.12&4967& -1.30&   4.37&  1.15&  1.11&39&7\\

[HB89] 0954+556&FOS H27 A-1&  2.58&  1.77&853&   8.6&  0.70&1782&  15.5&  0.36&1052& -1.30&   0.72&  1.21&  1.24&268&157\\

[HB89] 2216-038&FOS H27 A-1&  3.25&  1.15&-736&  10.4&  1.88&-341&  7.38&  0.66&-224& -1.30&   1.52&  0.84&  0.95&261&156\\
  3C 336&FOS H27 B-3&  2.36&  5.57&148&  11.4&  2.39&341&  6.96&  0.95&446&  0.56&  0.433&  1.11&  1.27&212&166\\
TON 0157&FOS H27 B-3&   9.8&  0.41&2384&  16.6&  0.61&-3876&   8.5&  0.14&1969& -2.31&    1.7&  1.42&  1.45&278&177\\
SBS 1148+549&FOS H27 A-1&  4.94&  1.31&-1258&    13&  0.84&-4957&  12.6&  1.16&-3499& -2.13&   5.66&  1.28&  1.20&279&177\\

[HB89] 2145+067&FOS H27 C-2&  1.81&  0.74&1518&  11.5&  1.70&934&  7.18&  0.58&1054& -0.20&   2.75&  0.85&  0.71&307&204\\

[HB89] 0355-483&FOS H27 A-1&   4.8&  1.51&-1401&  17.9&  1.08&1935&  3.19&  0.47&-972& -1.08&   2.57&  1.24&  1.03&270&180\\
TON 0153&FOS H27 C-2&  4.11&  0.39&-1527&  15.6&  0.86&-2517&  8.52&  0.41&-1782& -1.71&   6.18&  1.13&  0.84&293&183\\
PG 1254+047&FOS H27 C-2&  7.92&  1.70&-1409&  9.91&  1.82&-5922&  12.4&  2.66&-2503&  4.02&   1.91&  1.30&  1.13&308&185\\
PG 1248+401&FOS H27 B-2&  14.6&  1.78&-1305&  6.84&  0.53&-8625&  8.91&  0.99&-1068& -1.59&   2.87&  1.32&  1.56&290&174\\

[HB89] 2230+114&FOS H27 A-1&  4.44&  2.58&122&    17&  0.96&792&  4.09&  0.11&1148& -0.07&   1.43&  1.21&  1.06&315&199\\
LBQS 1229-0207&FOS H27 C-1&   2.3&  1.77&-256&  10.3&  2.66&-447&   6.3&  0.79&-87& -0.60&   1.66&  1.16&  1.41&196&159\\

[HB89] 2302+029&FOS H27 B-3&  1.04& -0.22&657&  16.9&  0.20&-4168&  21.5&  0.43&-2948& -0.27&   4.34&  1.38&  1.59&177&138\\
SBS 1317+520&FOS H27 A-1&  2.69&  1.41&-851&  12.5&  1.47&-101&  7.49&  0.41&529& -1.84&   2.73&  1.44&  1.48&318&172\\

[HB89] 1718+481&FOS H27 C-2&  3.58&  0.66&-413&  17.1&  0.68&-258&  5.98&  0.37&-593& -2.01&   15.1&  0.72&  0.66&191&182\\

[HB89] 0024+224&FOS H27 C-2&  6.84&  0.99&-1368&  10.7&  0.91&-3067&  14.4&  0.60&-2856& -1.13&   2.15&  0.99&  0.64&309&189\\
PG 1352+011&FOS H27 C-2&  2.33& -0.27&1665&  14.6&  1.13&-1837&  11.2&  0.55&-2431& -1.48&   3.68&  0.81&  0.76&274&192\\
PG 1206+459&FOS H27 C-2&  5.95&  0.33&-748&  11.7&  1.42&-382&  8.69&  1.10&-1039& -0.04&   4.62&  1.19&  0.89&222&175\\

[HB89] 1038+064&FOS H27 B-2&  4.68&  0.63&-159&  12.2&  0.73&-2786&  11.3&  0.64&-1458& -1.59&   2.76&  1.04&  1.30&306&231\\
PG 1241+176&FOS H27 C-2&   2.2&  1.36&919&  12.5&  1.15&2095&  3.92&  0.61&1074& -0.12&   3.59&  1.87&  1.52&284&210\\
PG 1008+133&FOS H27 C-2&  17.6&  0.69&628&  22.3&  0.08&-5647&  6.43&  0.20&-644& -1.33&   2.96&  1.63&  1.37&290&237\\

[HB89] 0454+039&FOS H27 B-3&  4.92&  1.14&16&  10.7&  0.89&-2152&  11.3&  0.74&-762& -1.28&   1.78&  1.86&  1.35&259&188\\
FBQS J1259487+342322&FOS H27 C-2&  2.65&  2.51&128&  12.3&  1.91&-443&  6.07&  0.86&166& -0.54&   1.11&  0.90&  0.52&353&244\\

[HB89] 0302-223&FOS H27 B-1&  6.36&  0.83&-1236&  32.4&  0.61&-694&  7.21&  0.31&-2153& -1.30&   2.28&  2.14&  1.87&227&157\\

[HB89] 0232-042&FOS H27 B-2&  4.87&  1.17&114&  16.7&  1.03&-725&  6.36&  0.39&267& -1.71&   2.97&  1.84&  1.07&378&158\\

[HB89] 1630+377&FOS H27 B-1&  4.05&  0.87&-605&  14.5&  1.14&-983&  7.76&  0.49&-200& -1.68&   3.48&  1.33&  1.08&338&140\\
PG 0117+213&FOS H27 B-2&  6.83&  0.54&-658&  20.9&  0.85&2026&  1.64&  0.13&93& -1.06&   3.76&  1.67&  1.71&260&69\\

[HB89] 0743-673&FOS H27 C-2&  3.83&  3.99&597&  14.2&  0.69&-495&   8.1&  0.34&39& -0.65&   1.98&  1.19&  1.07&285&111\\


==> table3.tex <==
MRK 0335&FOS H13 B-3&  2.46&  8.92&0&  8.12&  2.60&0&  5.23&  0.97&0& -1.30&   77.4&  1.24&  0.88&199&177\\
SBS 1626+554&FOS H13 B-3&  4.24&  1.48&0&  20.6&  1.41&0&  4.71&  0.29&0& -1.30&   21.8&  1.27&  1.24&326&217\\
PG 0026+129&FOS H13 B-3&  6.38&  3.47&0&  2.87&  7.31&0&  11.8&  1.09&0& -1.30&   19.6&  1.20&  1.26&311&199\\
  3C 273&FOS H13 A-1&  3.93&  0.77&0&  12.1&  0.74&0&  7.88&  0.32&0& -1.30&    269&  0.76&  0.79&372&204\\
  3C 273&FOS H13 B-3&  3.79&  0.96&0&  16.5&  0.62&0&  8.39&  0.18&0& -1.30&    269&  1.14&  1.08&354&204\\
  3C 273&FOS H13 B-1&  3.92&  0.96&0&  16.7&  0.57&0&  7.99&  0.19&0& -1.30&    282&  1.15&  1.04&352&203\\
  3C 273&FOS H13 C-2&  4.47&  0.85&0&  17.1&  0.56&0&  7.71&  0.19&0& -1.30&    279&  1.03&  0.88&317&160\\
  3C 273&FOS H13 B-2&  4.64&  0.76&0&  17.2&  0.57&0&  8.73&  0.20&0& -1.30&    271&  0.83&  0.82&355&203\\
PG 1322+659&FOS H13 B-3&  5.11&  3.03&0&  15.6&  0.83&0&  6.92&  0.78&0& -1.30&   9.19&  2.63&  1.51&279&194\\
PG 1116+215&FOS H13 C-2&  5.11&  1.11&0&  25.1&  0.86&0&  4.86&  0.25&0& -1.30&   53.3&  0.88&  0.58&362&219\\

[HB89] 1427+480&FOS H13 B-3&  3.53&  5.04&0&    10&  1.75&0&  7.31&  0.68&0& -1.30&   7.89&  1.32&  1.08&350&110\\
PG 0953+414&FOS H13 C-2&  5.26&  2.27&0&  22.6&  1.20&0&  4.09&  0.39&0& -1.30&   17.1&  1.35&  0.69&396&110\\

[HB89] 1156+213&FOS H19 B-3&  2.96&  4.29&0&  17.1&  1.43&0&  5.59&  0.36&0& -1.30&   3.15&  0.87&  0.78&248&156\\

[HB89] 1425+267&FOS H19 B-3&  8.78&  2.16&0&    28&  0.97&0&  1.66&  0.17&0& -1.30&   3.82&  1.63&  0.90&271&185\\
HS 0624+6907&FOS H19 B-2&  16.5&  0.77&0&  16.5&  1.39&0&  5.76&  0.76&0& -1.30&     15&  0.90&  0.76&252&133\\

[HB89] 1543+489&FOS H19 B-3&  19.8&  0.30&0&  19.8&  1.30&0&  1.24&  0.43&0& -1.30&   5.55&  1.55&  0.99&273&149\\
  3C 215&FOS H19 A-1&  8.26&  4.31&0&  22.4&  1.18&0&  22.1&  0.69&0& -1.30&  0.779&  0.65&  0.54&339&197\\
LBQS 1230+0947&FOS H19 A-1&  7.18&  2.59&0&  7.18&  2.99&0&  9.81&  1.67&0& -1.30&   6.02&  1.11&  1.33&337&175\\

[HB89] 1049+616&FOS L15 C-1&    10&  1.21&0&  32.3&  0.80&0&  7.24&  0.24&0& -1.30&   5.33&  0.98&  0.68&61&39\\

[HB89] 2308+098&FOS H19 B-3&  4.04&  2.30&0&  30.8&  1.24&0&  1.32&  0.19&0& -1.30&   5.98&  0.71&  0.57&330&197\\
PG 0003+158&FOS H19 C-2&  4.64&  1.93&0&  19.5&  1.44&0&5.85e+07&  0.06&0& -1.30&   11.3&  1.28&  0.51&327&202\\
FBQS J0745416+314256&FOS H19 C-2&  6.21&  0.81&0&  19.8&  1.58&0&  5.28&  0.09&0& -1.30&   5.57&  0.84&  0.63&350&214\\

[HB89] 2112+059 NED01&FOS H19 C-2&  19.8&  0.32&0&  19.8&  1.25&0&  2.53& -0.15&0& -1.30&   5.97&  0.97&  0.59&351&181\\
SBS 1259+593&FOS H19 C-2& 0.368& 12.43&0&  18.5&  0.86&0& 0.659& -0.10&0& -1.30&   11.1&  0.76&  0.85&353&216\\

[HB89] 2128-123&FOS H19 C-2&  7.99&  1.81&0&  30.3&  1.22&0&  -2.8&  0.04&0& -1.30&   8.67&  1.76&  1.88&226&178\\

[HB89] 0850+440&FOS H19 C-2&   3.4&  1.75&0&  16.2&  0.73&0&  6.47&  0.36&0& -1.30&   4.72&  0.43&  0.59&341&191\\
FBQS J0958209+322402&FOS H19 C-2&  3.98&  0.57&0&  33.9&  0.61&0&  1.12&  0.15&0& -1.30&   4.66&  0.32&  0.61&337&224\\

[HB89] 0015+162&FOS H19 B-3&  3.19&  1.78&0&  17.7&  1.17&0&  6.99&  0.49&0& -1.30&  0.444&  0.98&  1.09&346&228\\
  3C 334&FOS H19 C-2&  13.3&  0.88&0&  47.7&  0.58&0&  22.9& -0.00&0& -1.30&   5.05&  0.89&  1.01&350&227\\
NGC 2841 UB3&FOS H19 C-2&  2.92&  0.70&0&  17.8&  0.94&0&  7.63&  0.29&0& -1.30&    5.9&  1.00&  0.98&352&211\\

[HB89] 1136-135&FOS H19 C-2&    11&  1.32&0&  46.8&  0.60&0&  1.68&  0.32&0& -1.30&   4.45&  1.29&  0.92&352&230\\

[HB89] 0405-123&FOS H19 C-2&  5.61&  1.68&0&  24.3&  1.14&0&  3.28&  0.22&0& -1.30&   15.8&  1.32&  0.86&336&210\\

[HB89] 0439-433&FOS H19 C-2&  5.37&  2.03&0&  27.2&  1.00&0&   2.7&  0.18&0& -1.30&   3.53&  1.39&  0.86&340&224\\
FBQS J1010275+413238&FOS H19 C-2&  5.08&  2.90&0&  26.9&  1.46&0&  3.99&  0.37&0& -1.30&   6.32&  2.09&  1.46&338&200\\
  3C 095&FOS H19 C-2&  12.4&  0.75&0&    36&  0.55&0&  2.28&  0.10&0& -1.30&   9.19&  0.96&  1.05&355&237\\
PG 0044+030&FOS H19 C-2&  2.69&  2.53&0&  21.1&  1.68&0&   9.8&  0.28&0& -1.30&   3.68&  0.69&  0.62&390&238\\

[HB89] 2243-123&FOS H19 C-2&  3.97&  1.02&0&  22.4&  1.23&0&  4.38& -0.02&0& -1.30&   4.41&  1.69&  0.88&392&239\\

[HB89] 1104+167&FOS H19 C-2&  5.27&  1.23&0&  20.3&  1.67&0&  5.22&  0.04&0& -1.30&   7.95&  1.22&  1.22&365&239\\
  3C 263&FOS H19 A-1&  6.34&  1.87&0&    22&  1.12&0&  3.31&  0.35&0& -1.30&   6.16&  1.22&  1.16&395&242\\
  3C 263&FOS H19 C-2&  6.09&  1.32&0&  26.6&  1.01&0&  3.37& -0.21&0& -1.30&   7.06&  1.68&  0.68&374&240\\
  3C 057&FOS H19 B-2&  6.63&  1.22&0&  18.6&  0.27&0&   6.5&  0.45&0& -1.30&    6.9&  2.53&  1.37&376&235\\

[HB89] 2344+092&FOS H19 C-2&  2.94&  1.48&0&  16.9&  1.29&0&  5.78&  0.31&0& -1.30&   3.62&  1.42&  1.23&347&237\\

[HB89] 0923+392&FOS H19 A-1&  6.99&  2.60&0&  15.4&  0.90&0&  9.03&  0.47&0& -1.30&   4.79&  0.97&  1.00&385&189\\

[HB89] 2352-342&FOS H19 C-2&  9.04&  2.88&0&  28.5&  0.33&0&  8.17&  0.62&0& -1.30&   4.46&  1.97&  0.90&339&227\\

[HB89] 1354+195&FOS H19 C-2&  4.72&  2.16&0&  21.1&  1.24&0&  3.43&  0.20&0& -1.30&   3.55&  1.54&  0.89&414&160\\

[HB89] 1637+574&FOS H19 A-1&  4.55&  1.60&0&  13.7&  0.92&0&  7.28&  0.50&0& -1.30&      3&  1.16&  0.87&422&128\\

[HB89] 1538+477&FOS H19 C-2&  7.39&  1.99&0&  20.3&  1.09&0&  7.37&  0.30&0& -1.30&   5.89&  2.42&  1.80&288&112\\
2MASSI J1003067+681316&FOS H19 C-2& 0.469& 14.27&0&  18.5&  0.64&0&  13.1&  0.51&0& -1.30&   2.78&  1.11&  1.16&387&111\\
  3C 110&FOS H19 B-3&  6.17&  0.74&0&  20.4&  1.27&0&  9.27&  0.21&0& -1.30&   4.32&  1.40&  1.19&426&112\\
LBQS 0102-2713&FOS H19 B-3&  1.74&  6.46&0&  17.2&  1.49&0&     8&  0.40&0& -1.30&   1.33&  2.24&  2.38&346&75\\
FBQS J1253175+310550&FOS H19 B-3&  5.52&  0.36&0&    18&  1.52&0&  5.43&  0.33&0& -1.30&   2.68&  3.76&  2.60&335&66\\
  3C 286&FOS L15 A-1&  3.54&  0.18&0&  15.7&  0.69&0&  5.52&  0.08&0& -1.30&   1.79&  1.02&  1.84&75&12\\
 3C 4543&FOS H27 C-2&-0.211&-20.86&0&    11&  0.60&0&  3.16&  0.26&0& -1.30&   2.78&  0.62&  0.78&217&146\\
 3C 4543&FOS H27 A-1&  3.87&  2.00&0&  19.9&  0.56&0&  3.04&  0.32&0& -1.30&   1.59&  1.13&  1.39&212&141\\

[HB89] 0107-156&FOS H27 B-3&   1.6& 10.95&0&  17.3&  1.60&0&  7.44&  0.10&0& -1.30&   0.73&  1.01&  0.96&191&126\\

[HB89] 1252+119&FOS H27 C-2&  3.48&  0.74&0&  17.2&  0.79&0&  5.96&  0.30&0& -1.30&   2.24&  0.90&  0.85&264&155\\
LBQS 0253-0138&FOS H27 A-1&  2.25&  2.86&0&    18&  0.80&0&  9.04&  0.28&0& -1.30&   2.22&  1.21&  1.34&267&146\\

[HB89] 2340-036&FOS H27 C-2&  6.62&  1.90&0&  30.6&  0.81&0&  1.07& -0.34&0& -1.30&   4.37&  1.15&  1.11&39&7\\

[HB89] 0954+556&FOS H27 A-1&  4.21&  2.95&0&  25.7&  0.80&0&  5.57& -0.05&0& -1.30&   0.72&  1.21&  1.24&268&157\\

[HB89] 2216-038&FOS H27 A-1&  6.72&  0.83&0&  14.2&  1.06&0&  6.84&  0.50&0& -1.30&   1.52&  0.84&  0.95&261&156\\
  3C 336&FOS H27 B-3&  5.29&  1.60&0&  23.5&  1.25&0&  1.47&  0.22&0& -1.30&  0.512&  1.11&  1.27&212&166\\
TON 0157&FOS H27 B-3& -1.19&-125.44&0&  12.4&  0.82&0&  14.1&  0.24&0& -1.30&   1.55&  1.42&  1.45&278&177\\
SBS 1148+549&FOS H27 A-1&  6.08& -0.03&0&  19.1&  1.66&0&  25.5& -0.00&0& -1.30&   5.23&  1.28&  1.20&279&177\\

[HB89] 2145+067&FOS H27 C-2&  2.93& 10.51&0&   9.5&  1.80&0&  11.9&  0.60&0& -1.30&   3.03&  0.85&  0.71&307&204\\

[HB89] 0355-483&FOS H27 A-1&  1.76&  4.44&0&  18.4&  1.16&0&  7.46&  0.28&0& -1.30&   2.63&  1.24&  1.03&270&180\\
TON 0153&FOS H27 C-2&   -13&-349.20&0&    13&349.86&0&     2& -0.06&0& -1.30&   5.96&  1.13&  0.84&293&183\\
PG 1254+047&FOS H27 C-2& 0.508& 11.74&0&  19.2&  1.26&0&  2.02&  0.22&0& -1.30&   3.25&  1.30&  1.13&308&185\\
PG 1248+401&FOS H27 B-2&  16.6&  0.81&0&  16.6&  1.29&0&  6.33&  0.47&0& -1.30&   2.78&  1.32&  1.56&290&174\\

[HB89] 2230+114&FOS H27 A-1&   2.9&  2.00&0&  8.99&  1.87&0&  7.67&  0.34&0& -1.30&   1.58&  1.21&  1.06&315&199\\
LBQS 1229-0207&FOS H27 C-1&  6.68&  1.69&0&  26.5&  0.75&0&  4.04&  0.27&0& -1.30&   1.78&  1.16&  1.41&196&159\\

[HB89] 2302+029&FOS H27 B-3&  1.69&  1.32&0&  18.9&  0.31&0&  12.9&  0.15&0& -1.30&    4.8&  1.38&  1.59&177&138\\
SBS 1317+520&FOS H27 A-1&  5.21&  0.88&0&  23.9&  0.96&0&1.83e+07&  0.05&0& -1.30&   2.63&  1.44&  1.48&318&172\\

[HB89] 1718+481&FOS H27 C-2&   2.6&  0.58&0&  17.7&  0.78&0&  7.65&  0.33&0& -1.30&   14.2&  0.72&  0.66&191&182\\

[HB89] 0024+224&FOS H27 C-2&   4.1&  0.62&0&  18.6&  0.80&0&  8.91&  0.10&0& -1.30&   2.18&  0.99&  0.64&309&189\\
PG 1352+011&FOS H27 C-2& 0.612&  8.35&0&  18.4&  1.22&0&0.0918& -0.07&0& -1.30&   3.61&  0.81&  0.76&274&192\\
PG 1206+459&FOS H27 C-2& 0.693& 11.64&0&    17&  1.42&0&   5.9&  0.47&0& -1.30&   5.16&  1.19&  0.89&222&175\\

[HB89] 1038+064&FOS H27 B-2&  3.84&  0.44&0&  17.4&  0.78&0&  7.76&  0.33&0& -1.30&   2.68&  1.04&  1.30&306&231\\
PG 1241+176&FOS H27 C-2&  4.42& -0.26&0&  7.17&  1.54&0&  17.7&  0.64&0& -1.30&   4.01&  1.87&  1.52&284&210\\
PG 1008+133&FOS H27 C-2&  1.54&  3.58&0&  16.6&  0.87&0&  6.83&  0.23&0& -1.30&   2.93&  1.63&  1.37&290&237\\

[HB89] 0454+039&FOS H27 B-3&  4.17&  1.22&0&  29.1&  0.72&0&  6.15&  0.20&0& -1.30&    1.8&  1.86&  1.35&259&188\\
FBQS J1259487+342322&FOS H27 C-2&  4.61&  1.89&0&  24.4&  0.95&0&  3.91&  0.36&0& -1.30&   1.19&  0.90&  0.52&353&244\\

[HB89] 0302-223&FOS H27 B-1&  1.25& 10.20&0&    24&  0.93&0&  7.22&  0.04&0& -1.30&   2.28&  2.14&  1.87&227&157\\

[HB89] 0232-042&FOS H27 B-2&  6.21&  1.54&0&  19.8&  0.65&0&   6.8&  0.38&0& -1.30&   2.89&  1.84&  1.07&378&158\\

[HB89] 1630+377&FOS H27 B-1&  1.82&  7.86&0&  19.8&  0.94&0&  5.79&  0.25&0& -1.30&    3.4&  1.33&  1.08&338&140\\
PG 0117+213&FOS H27 B-2&  1.57& 22.69&0&  23.5&  0.92&0&  6.24&  0.16&0& -1.30&   3.82&  1.67&  1.71&260&69\\

[HB89] 0743-673&FOS H27 C-2&  3.52&  1.14&0&  8.73&  1.42&0&  7.32&  0.38&0& -1.30&   2.05&  1.19&  1.07&285&111\\

